Dual-Input Dynamic Convolution for Positron Range Correction in PET Image Reconstruction

Positron range (PR) blurring degrades positron emission tomography (PET) image resolution, particularly for high-energy emitters like gallium-68 (68 Ga). We introduce Dual-Input Dynamic Convolution (DDConv), a novel computationally efficient approach trained with voxel-specific PR point spread functions (PSFs) from Monte Carlo (MC) simulations and designed to be utilized within an iterative reconstruction algorithm to perform PR correction (PRC). By dynamically inferring local blurring kernels through a trained convolutional neural network (CNN), DDConv captures complex tissue interfaces more accurately than prior methods. Additionally, it also computes the transpose operator, ensuring consistency within iterative PET reconstruction. Comparisons with a state-of-the-art, tissue-dependent correction confirm the advantages of DDConv in recovering higher-resolution details in heterogeneous regions, including bone-soft tissue and lung-soft tissue boundaries. Experiments across digital phantoms and MC-simulated data show that DDConv offers near-MC accuracy and outperforms the state-of-the-art technique, namely spatially-variant and tissue-dependent (SVTD), especially in areas with complex material interfaces. Results from real phantom experiments further confirm DD-Conv's robustness and practical applicability: while both DD-Conv and SVTD performed similarly in homogeneous soft-tissue regions, DDConv provided more accurate activity recovery and sharper delineation at heterogeneous lung-soft tissue interfaces. Our code available at https://github.com/mellak/ddconv-prc.

==> images/RealPhantom.tex <==
\begin{figure}[htbp]
  \centering
  % 2x2 grid of grey placeholder images
  \begin{tabular}{cc}
    \subfloat[Materials\label{subfig:materials}]{%
      \colorbox{gray!40}{%
        \parbox[c][3cm][c]{0.45\linewidth}{\centering\textcolor{white}{Placeholder}}%
      }%
    } &
    \subfloat[NOPRC\label{subfig:noprc}]{%
      \colorbox{gray!40}{%
        \parbox[c][3cm][c]{0.45\linewidth}{\centering\textcolor{white}{Placeholder}}%
      }%
    } \\
    \subfloat[SVTD\label{subfig:svtd}]{%
      \colorbox{gray!40}{%
        \parbox[c][3cm][c]{0.45\linewidth}{\centering\textcolor{white}{Placeholder}}%
      }%
    } &
    \subfloat[DDConv\label{subfig:ddconv}]{%
      \colorbox{gray!40}{%
        \parbox[c][3cm][c]{0.45\linewidth}{\centering\textcolor{white}{Placeholder}}%
      }%
    }
  \end{tabular}
  
  \vspace{0.5cm}
  
  % Centered plot with random curves
  \begin{tikzpicture}
    \begin{axis}[
      width=0.8\linewidth,
      height=0.4\linewidth,
      xlabel={X-axis},
      ylabel={Y-axis},
      title={Random Plot},
      grid=both
    ]
      \addplot+[blue, mark=none, domain=0:10, samples=50] {rand*10};
      \addplot+[red, mark=none, domain=0:10, samples=50] {rand*10};
      \addplot+[green, mark=none, domain=0:10, samples=50] {rand*10};
    \end{axis}
  \end{tikzpicture}
  
  \caption{2×2 configuration of placeholder images for Materials, NOPRC, SVTD and DDConv with a centered plot below displaying random curves. \textcolor{red}{I need to add images, wiating just for new reconstructions here}}

  \label{fig:Real_Phantom}
\end{figure}


==> images/real_attenuation.tex <==
\newcommand{\iter}{01} % <-- set iteration number here

\begin{figure}[!t]
  \centering
  \subfloat[Tumor 1\label{subfig:attenuation_t1}]{%
    \includegraphics[width=0.49\linewidth]{images/RealPhantom/ct_t1_it01.png}%
  }\hfill
  \subfloat[Tumor 2\label{subfig:tattenuation_t2}]{%
    \includegraphics[width=0.49\linewidth]{images/RealPhantom/ct_t2_it01.png}%
  }
  \caption{
    Attenuation map slices. The red dots indicate the positions of the activity centers,  
    while the green boxes denote the $11\times11\times11$\,voxel regions of interest used for analysis.}

\end{figure}

==> images/real_reconstructions.tex <==
% Command for images without the extra vertical line
\newcommand{\spiedimage}[2]{%  % #1 = image path, #2 = iteration number
  \begin{tikzpicture}[spy using outlines={circle, magnification=2, size=0.5cm, connect spies, red}]
    % Place the image inside a node.
    \node (img) {\includegraphics[width=0.18\linewidth]{#1}};
    
    % Add iteration number to top left of image
    \node[text=vividorange, font=\footnotesize\bfseries, anchor=north west] 
         at (img.north west) {iter. #2};
    
    % Set the spy overlay.
    \spy [vividorange] on ($(img.center)+(-0.12,-0.2)$)
         in node [fill=white] at ($(img.east)+(-0.5cm,-0.7cm)$);
  \end{tikzpicture}%
}

\newcommand{\spiedimagelast}[2]{%  % #1 = image path, #2 = iteration number
  \begin{tikzpicture}[spy using outlines={circle, magnification=2, size=0.5cm, connect spies, red}]
    % Place the image inside a node.
    \node (img) {\includegraphics[width=0.18\linewidth]{#1}};
    
    % Add iteration number to top left of image
    \node[text=vividorange, font=\footnotesize\bfseries, anchor=north west] 
         at (img.north west) {iter. #2};
    
    % Draw a vertical green line at the desired offset.
    \draw[green, line width=0.5pt]
         ($(img.center)+(-0.12,-0.2)+(0,0.20)$) -- ($(img.center)+(-0.12,-0.2)+(0,-0.19)$);
         
    % Then apply the spy overlay.
    \spy [vividorange] on ($(img.center)+(-0.12,-0.2)$)
         in node [fill=white] at ($(img.east)+(-0.5cm,-0.7cm)$);
  \end{tikzpicture}%
}

\begin{figure*}[htbp]
  \centering
  \begin{minipage}[t]{0.9\textwidth}
    % Row 1: NoPRC images
    \begin{minipage}{0.03\linewidth}
      \centering
      \rotatebox{90}{\tiny no PRC}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
      \centering
      \spiedimage{images/RealReconstructions/nopr_it24.png}{24}%
      \spiedimage{images/RealReconstructions/nopr_it48.png}{48}%
      \spiedimage{images/RealReconstructions/nopr_it72.png}{72}%
      \spiedimage{images/RealReconstructions/nopr_it96.png}{96}%
      % For iteration 120, use the command that draws the vertical green line.
      \spiedimagelast{images/RealReconstructions/nopr_it120.png}{120}%
    \end{minipage}\\[3mm]
    
    % Row 2: SVTD images
    \begin{minipage}{0.03\linewidth}
      \centering
      \rotatebox{90}{\tiny SVTD}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
      \centering
      \spiedimage{images/RealReconstructions/smns_it24.png}{24}%
      \spiedimage{images/RealReconstructions/smns_it48.png}{48}%
      \spiedimage{images/RealReconstructions/smns_it72.png}{72}%
      \spiedimage{images/RealReconstructions/smns_it96.png}{96}%
      \spiedimagelast{images/RealReconstructions/smns_it120.png}{120}%
    \end{minipage}\\[3mm]
    
    % Row 3: DDConv images
    \begin{minipage}{0.03\linewidth}
      \centering
      \rotatebox{90}{\tiny DDConv}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
      \centering
      \spiedimage{images/RealReconstructions/myprc_it24.png}{24}%
      \spiedimage{images/RealReconstructions/myprc_it48.png}{48}%
      \spiedimage{images/RealReconstructions/myprc_it72.png}{72}%
      \spiedimage{images/RealReconstructions/myprc_it96.png}{96}%
      \spiedimagelast{images/RealReconstructions/myprc_it120.png}{120}%
    \end{minipage}
  \end{minipage}
  \caption{Experiment 3---\Ac{EM}-reconstructed images (patient data) with no \ac{PRC}, \ac{SVTD} and \ac{DDConv} at different iterations.}
  \label{fig:res_real_phantom_reconstructions}
\end{figure*}

==> images/xcat_reconstructions.tex <==


%%

\newcommand{\xcatImgSpy}[2]{% % #1 = image path, #2 = iteration number
\begin{tikzpicture}[spy using outlines={circle, magnification=2, size=0.5cm, connect spies, vividorange}]
  % Place the image inside a node.
  \node (img) {\includegraphics[width=0.2\linewidth]{#1}};
  
  % Add iteration number to top left of image
  \node[text=vividorange, font=\footnotesize\bfseries, anchor=north west] 
       at (img.north west) {iter. #2};
  
  % Apply the spy overlay.
  \spy [vividorange] on ($(img.south east)+(-2.1,0.65)$) 
       in node [left] at ($(img.north west)+(0.8,-1.3)$);
\end{tikzpicture}%
}

\newcommand{\xcatImgSpyLast}[2]{% % #1 = image path, #2 = iteration number
\begin{tikzpicture}[spy using outlines={circle, magnification=2, size=0.5cm, connect spies, vividorange}]
  % Place the image inside a node.
  \node (img) {\includegraphics[width=0.2\linewidth]{#1}};
  
  % Add iteration number to top left of image
  \node[text=vividorange, font=\footnotesize\bfseries, anchor=north west] 
       at (img.north west) {iter. #2};
  
  % Apply the spy overlay.
  \spy [vividorange] on ($(img.south east)+(-2.1,0.65)$) 
       in node [left] at ($(img.north west)+(0.8,-1.3)$);
  
  % Add green line
  \draw[green, line width=0.5pt] (-0.43,-0.1) -- (-0.43,-0.35);
\end{tikzpicture}%
}

\begin{figure*}[htbp]
\centering
\begin{minipage}[t]{0.9\textwidth}
  % Row 1: NoPRC images
  \begin{minipage}{0.03\linewidth}
    \centering
    \rotatebox{90}{\tiny No PRC}
  \end{minipage}
  \begin{minipage}{0.95\linewidth}
    \centering
    \xcatImgSpy{images/XCatReconstructions/nopr_it24.png}{24}%
    \xcatImgSpy{images/XCatReconstructions/nopr_it48.png}{48}%
    \xcatImgSpy{images/XCatReconstructions/nopr_it72.png}{72}%
    \xcatImgSpy{images/XCatReconstructions/nopr_it96.png}{96}%
    \xcatImgSpyLast{images/XCatReconstructions/nopr_it120.png}{120}%
  \end{minipage}\\[3mm]
  
  % Row 2: SVTD images
  \begin{minipage}{0.03\linewidth}
    \centering
    \rotatebox{90}{\tiny SVTD}
  \end{minipage}
  \begin{minipage}{0.95\linewidth}
    \centering
    \xcatImgSpy{images/XCatReconstructions/smns_it24.png}{24}%
    \xcatImgSpy{images/XCatReconstructions/smns_it48.png}{48}%
    \xcatImgSpy{images/XCatReconstructions/smns_it72.png}{72}%
    \xcatImgSpy{images/XCatReconstructions/smns_it96.png}{96}%
    \xcatImgSpyLast{images/XCatReconstructions/smns_it120.png}{120}%
  \end{minipage}\\[3mm]
  
  % Row 3: DDConv images
  \begin{minipage}{0.03\linewidth}
    \centering
    \rotatebox{90}{\tiny DDConv}
  \end{minipage}
  \begin{minipage}{0.95\linewidth}
    \centering
    \xcatImgSpy{images/XCatReconstructions/myprc_it24.png}{24}%
    \xcatImgSpy{images/XCatReconstructions/myprc_it48.png}{48}%
    \xcatImgSpy{images/XCatReconstructions/myprc_it72.png}{72}%
    \xcatImgSpy{images/XCatReconstructions/myprc_it96.png}{96}%
    \xcatImgSpyLast{images/XCatReconstructions/myprc_it120.png}{120}%
  \end{minipage}
\end{minipage}
\caption{Experiment 2---\Ac{EM}-reconstructed images (\ac{MC}-simulated data) with no \ac{PRC}, \ac{SVTD} and \ac{DDConv} at different iterations.}
\label{fig:xcat_Reconstructions}
\end{figure*}
